Poisson-like cohomologies associated with some Lie superalgebras

The concept of Poisson cohomology groups associated with Poisson manifolds is a part of the theory of Lie superalgebras of vector fields. Therefore, we abstracted them as Poisson-like cohomology groups for general Lie superalgebras. In doing so, we obtained a generalization of the concept of the Euler number. For the Lie superalgebras of differential forms on a manifold, we found the de Rham cohomology groups match with the Poisson-like cohomology groups in the special case. In order to understand the development of the discussion, we presented some simple examples and show ideas of how our discussion unfolds.

==> km-env-eng.tex <==
\usepackage{ntheorem}

{
\theoremheaderfont{\bfseries }
\theorembodyfont{\rmfamily}
% \theoremstyle{break}  
\theoremstyle{plain}  
% \newtheorem{nota}{\bfseries  記号}[section]
%\newtheorem{defn}{\bfseries  定義}[section]
%\newtheorem{prop}{\bfseries  命題}[section]
%\newtheorem{exam}{\bfseries  例}[section]
%\newtheorem{remark}{\bfseries  注意}[section]
\newtheorem{prob}{\bfseries  練習問題}[section]
%
\theoremstyle{plain}  
\newtheorem{defn}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{exam}{\bfseries  Example}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[theorem]{Proposition}
\newtheorem*{prop-non}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{propfid}{Proposition \ref{originrel}}
}






\newcommand{\me}{\mathbf{e}}
\newcommand{\mf}{\mathbf{f}}
%\newcommand{\mH}{\mathbb{H}} %Use in Math-mode
%\newcommand{\mC}{{\mbox{\bfseries  C}}} %Use in Math-mode
%\newcommand{\mC}{\mathbb{C}} %Use in Math-mode
%\newcommand{\mZ}{{\mbox{\bfseries  Z}}} %Use in Math-mode
%\newcommand{\pdel}{\partial} %Use in Math-mode
%\newcommand{\bm}[1]{\mbox{\boldmath $#1$}} %Use in Math-mode
%\renewcommand{\frak}{\mathfrak}
%\renewcommand{\[}{$$} \renewcommand{\]}{$$} 
%\newcommand{\SbtS}[2]{[#1,#2]_{\text{\footnotesize S}}} %Use in Math-ode 
%\newcommand{\Alt}[3]{{\langle{#1}\rangle^{#2}_{#3}}  %Use in Math-mode 
%\newcommand{\Alt}[3]{{}^{#2}\langle{#1}\rangle_{#3}}  %Use in Math-mode 

\newcommand{\yokob}{\par\medskip\noindent\makebox[\paperwidth]{\hrulefill}\par}
\newcommand{\yokoe}{\par\noindent\makebox[\paperwidth]{\hrulefill}\par\medskip}
\newcommand{\aida}{\par\noindent\makebox[\textwidth]{\hrulefill}\par}
%

\newcommand{\vare}{\varepsilon} %Use in Math-mode
\newcommand{\qed}{\hfill \rule{1ex}{1.5ex}\par}
\renewcommand{\[}{$$} \renewcommand{\]}{$$}

%\newcommand{\backl}{\mathbin
% {\vrule width1.5ex height.4pt\vrule height1.5ex}}


%\newcommand{\frakg}{{\mathfrak g}}
\newcommand{\frakl}{{\mathfrak l}}
%\newcommand{\frakh}{{\mathfrak h}}
\newcommand{\frakm}{{\mathfrak m}}
\newcommand{\fraks}{{\mathfrak s}}
\newcommand{\frako}{{\mathfrak o}}
\newcommand{\frakp}{{\mathfrak p}}
\newcommand{\fraku}{{\mathfrak u}}

\newcommand{\frakgl}{{\mathfrak g}{\mathfrak l}}
%\newcommand{\fraksl}{{\mathfrak s}{\mathfrak l}}
%\newcommand{\frakso}{{\mathfrak s}{\mathfrak o}}
%\newcommand{\fraksu}{{\mathfrak s}{\mathfrak u}}
%\newcommand{\fraksp}{{\mathfrak s}{\mathfrak p}}


\endinput 


==> km-env-j.tex <==
\usepackage{theorem}


\theoremstyle{plain}  
% \theoremstyle{break}  
\theoremheaderfont{\normalfont\bfseries}
\theorembodyfont{\rmfamily}
\newtheorem{nota}{記号}[section]
\newtheorem{defn}{定義}[section]
\newtheorem{prop}{命題}[section]
\newtheorem{exam}{例}[section]
\newtheorem{remark}{注意}[section]
\newtheorem{prob}{問題}[section]
\newtheorem{kmComment}{コメント}[section]
%
\theoremstyle{plain}  
\newtheorem{definition}{Definition}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{exam}{\textbf{Example}}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{thm}{定理}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[thm]{補題}
\newtheorem{cor}[thm]{系}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propfid}{Proposition \ref{originrel}} 





\newcommand{\me}{\mathbf{e}}
\newcommand{\mf}{\mathbf{f}}
%\newcommand{\bm}[1]{\mbox{\boldmath $#1$}} %Use in Math-mode
%\renewcommand{\frak}{\mathfrak}
%\renewcommand{\[}{$$} \renewcommand{\]}{$$} 
%\newcommand{\SbtS}[2]{[#1,#2]_{\text{\footnotesize S}}} %Use in Math-ode 
%\newcommand{\Alt}[3]{{\langle{#1}\rangle^{#2}_{#3}}  %Use in Math-mode 
%\newcommand{\Alt}[3]{{}^{#2}\langle{#1}\rangle_{#3}}  %Use in Math-mode 

\newcommand{\yokob}{\par\medskip\noindent\makebox[\paperwidth]{\hrulefill}\par}
\newcommand{\yokoe}{\par\noindent\makebox[\paperwidth]{\hrulefill}\par\medskip}
\newcommand{\aida}{\par\noindent\makebox[\textwidth]{\hrulefill}\par}
%

\newcommand{\vare}{\varepsilon} %Use in Math-mode
\newcommand{\qed}{\hfill \rule{1ex}{1.5ex}\par}
\renewcommand{\[}{$$} \renewcommand{\]}{$$}

\newcommand{\backl}{\mathbin{\vrule width1.5ex height.4pt\vrule
 height1.5ex}}


\newcommand{\frakl}{\mathfrak{l}}
\newcommand{\frakm}{\mathfrak{m}}
\newcommand{\fraks}{\mathfrak{s}}
\newcommand{\frako}{\mathfrak{o}}
\newcommand{\frakp}{\mathfrak{p}}
\newcommand{\fraku}{\mathfrak{u}}

\newcommand{\frakgl}{\mathfrak{gl}}
\newcommand{\frakso}{\mathfrak{so}}
\newcommand{\fraksu}{\mathfrak{su}}

\endinput 


==> km-env-nthm.tex <==
%\input km-env-e.tex 
%\usepackage[amsthm]{ntheorem} 
\usepackage{ntheorem} 
{
\theoremheaderfont{\bfseries}
\theorembodyfont{\rmfamily}
%\theoremstyle{break}  
%\theoremstyle{plain}  
\newtheorem{nota}{\textbf{Notation}}[section]
\newtheorem{defn}{\textbf{Definition}}
\newtheorem{prop}{Proposition}[section]
\newtheorem{exam}{Example}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{prob}{Problem}[section]
\newtheorem{fact}{Fact}
%
%\theoremstyle{plain}  
\newtheorem{definition}{Definition}[section]
%\newtheorem{remark}{Remark}[section]
%\newtheorem{exam}{\textbf{Example}}[section]
\newtheorem{theorem}{Theorem}[section] 
\newtheorem{thm}{Theorem}[section]
\newtheorem*{thm-none}{Theorem}[section]
\newtheorem{kmProp}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{kmCor}[theorem]{Corollary}
\newtheorem{kmRemark}{Remark}[section]
\newtheorem{kmComment}{Comment}[section]
\newtheorem{propfid}{Proposition \ref{originrel}}
}




==> km-env-old.tex <==
%
%\theoremstyle{definition} % for AMSLATEX
%
\newtheorem{lemma}{Lemma}[section] 
%\newtheorem{prop}{Proposition}[section] %
\newtheorem{prop}{Proposition}[section]
%\newtheorem{cor}{Cor}[section] %
\newtheorem{cor}{Corollary}[section]
%\newtheorem{defn}{Defn}[section] %
\newtheorem{defn}{Definition}[section] 
\newtheorem{exam}{Example}[section]

\newtheorem{thm}[prop]{Theorem}
%
%
%% \theoremstyle{remark}  % for AMSLATEX
\newtheorem{remark}{\bf Remark}[section]
\newtheorem{fact}{\bf Fact}
% 

\newcommand{\me}{\mathbf{e}}
\newcommand{\mf}{\mathbf{f}}
\newcommand{\mZ}{{\mbox{\bf Z}}} %Use in Math-mode
\newcommand{\mQ}{{\mbox{\bf Q}}} %Use in Math-mode
\newcommand{\mR}{{\mbox{\bf R}}} %Use in Math-mode
\newcommand{\mC}{{\mbox{\bf C}}} %Use in Math-mode 
\newcommand{\pdel}{\partial} %Use in Math-mode
\newcommand{\yokob}{\par\medskip\noindent\makebox[\paperwidth]{\hrulefill}\par}
\newcommand{\yokoe}{\par\noindent\makebox[\paperwidth]{\hrulefill}\par\medskip}
\newcommand{\aida}{\par\noindent\makebox[\textwidth]{\hrulefill}\par}
%

\newcommand{\vare}{\varepsilon} %Use in Math-mode
\newcommand{\qed}{\hfill \rule{1ex}{1.5ex}\par}
\renewcommand{\[}{$$} \renewcommand{\]}{$$}

\newcommand{\backl}{\mathbin{\vrule width1.5ex height.4pt\vrule
 height1.5ex}}

\endinput 


==> km-env.tex <==
\usepackage{theorem}

{
\theoremheaderfont{\bfseries }
\theorembodyfont{\rmfamily}
% \theoremstyle{break}  
\theoremstyle{plain}  
\newtheorem{nota}{\bfseries  記号}[section]
\newtheorem{defn}{\bfseries  定義}[section]
\newtheorem{prop}{\bfseries  命題}[section]
\newtheorem{thm}{\bfseries 定理}[section]
\newtheorem{coro}[thm]{系}
% \newtheorem{exam}{\bfseries  例}[section]
% \newtheorem{remark}{\bfseries  注意}[section]
\newtheorem{prob}{\bfseries  練習問題}[section]
%
\theoremstyle{plain}  
\newtheorem{definition}{Definition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{exam}{\bfseries Example}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{propfid}{Proposition \ref{originrel}}
}






\newcommand{\me}{\mathbf{e}}
\newcommand{\mf}{\mathbf{f}}
%\newcommand{\mR}{\mathbb{R}} %Use in Math-mode
%\newcommand{\mH}{\mathbb{H}} %Use in Math-mode
%\newcommand{\mC}{{\mbox{\bfseries  C}}} %Use in Math-mode
%\newcommand{\mC}{\mathbb{C}} %Use in Math-mode
%\newcommand{\mZ}{{\mbox{\bfseries  Z}}} %Use in Math-mode
%\newcommand{\pdel}{\partial} %Use in Math-mode
%\newcommand{\bm}[1]{\mbox{\boldmath $#1$}} %Use in Math-mode
%\renewcommand{\frak}{\mathfrak}
%\renewcommand{\[}{$$} \renewcommand{\]}{$$} 
%\newcommand{\SbtS}[2]{[#1,#2]_{\text{\footnotesize S}}} %Use in Math-ode 
%\newcommand{\Alt}[3]{{\langle{#1}\rangle^{#2}_{#3}}  %Use in Math-mode 
%\newcommand{\Alt}[3]{{}^{#2}\langle{#1}\rangle_{#3}}  %Use in Math-mode 

\newcommand{\yokob}{\par\medskip\noindent\makebox[\paperwidth]{\hrulefill}\par}
\newcommand{\yokoe}{\par\noindent\makebox[\paperwidth]{\hrulefill}\par\medskip}
\newcommand{\aida}{\par\noindent\makebox[\textwidth]{\hrulefill}\par}
%

\newcommand{\vare}{\varepsilon} %Use in Math-mode
\newcommand{\qed}{\hfill \rule{1ex}{1.5ex}\par}
\renewcommand{\[}{$$} \renewcommand{\]}{$$}

%\newcommand{\backl}{\mathbin
% {\vrule width1.5ex height.4pt\vrule height1.5ex}}


%\newcommand{\frakg}{{\mathfrak g}}
\newcommand{\frakl}{{\mathfrak l}}
%\newcommand{\frakh}{{\mathfrak h}}
\newcommand{\frakm}{{\mathfrak m}}
\newcommand{\fraks}{{\mathfrak s}}
\newcommand{\frako}{{\mathfrak o}}
\newcommand{\frakp}{{\mathfrak p}}
\newcommand{\fraku}{{\mathfrak u}}

\newcommand{\frakgl}{{\mathfrak g}{\mathfrak l}}
%\newcommand{\fraksl}{{\mathfrak s}{\mathfrak l}}
%\newcommand{\frakso}{{\mathfrak s}{\mathfrak o}}
%\newcommand{\fraksu}{{\mathfrak s}{\mathfrak u}}
%\newcommand{\fraksp}{{\mathfrak s}{\mathfrak p}}











\endinput 

